UIEDP:Underwater Image Enhancement with Diffusion Prior

Underwater image enhancement (UIE) aims to generate clear images from low-quality underwater images. Due to the unavailability of clear reference images, researchers often synthesize them to construct paired datasets for training deep models. However, these synthesized images may sometimes lack quality, adversely affecting training outcomes. To address this issue, we propose UIE with Diffusion Prior (UIEDP), a novel framework treating UIE as a posterior distribution sampling process of clear images conditioned on degraded underwater inputs. Specifically, UIEDP combines a pre-trained diffusion model capturing natural image priors with any existing UIE algorithm, leveraging the latter to guide conditional generation. The diffusion prior mitigates the drawbacks of inferior synthetic images, resulting in higher-quality image generation. Extensive experiments have demonstrated that our UIEDP yields significant improvements across various metrics, especially no-reference image quality assessment. And the generated enhanced images also exhibit a more natural appearance.

==> tables/abla_IC.tex <==
\begin{table}
    \centering
    \begin{tabular}{lccccc}
    \toprule
    Method & \multicolumn{3}{c}{F1@\{10,25,50\}} & Edit  & Acc \\
    \midrule\midrule
    
    PLE & 72.2 & 69.0 & 57.3 & 64.4 & 76.6 \\
    Temp AGNES & 72.2 & 68.3 & 56.3 & 64.5 & 73.2 \\
    \midrule
    Li \textit{et al.} & 75.4  & 72.4  & 61.8  & 68.1  & 76.8 \\
    IC (Li \textit{et al.})  & 74.7 & 71.8 & 62.1 & 66.2 & 77.6 \\
    \midrule
    IC (Ours) & \textbf{76.0} & \textbf{73.2} & \textbf{63.7} & \textbf{68.5} & \textbf{78.5}\\
    
    \bottomrule
    \end{tabular}
    \caption{Comparison of supervision generated by different methods. The first two and the middle two rows represent that pseudo-labels are fixed and updated during training, respectively. \textit{IC (Li et al.)} refers to using the energy function to generate pseudo-labels for the ambiguous intervals in pseudo-label sequences during IC. \textit{IC (Ours)} is IC we propose.}
    \label{tab:abla_IC}
\end{table}
